Uncovering astrometric black hole binaries with massive main-sequence companions with Gaia

The hunt for compact objects is on. Rarely seen massive binaries with a compact object are a crucial phase in the evolution towards compact object mergers. In Gaia data release 3 (DR3), the first Gaia astrometric orbital solutions for binary sources will become available. We investigate how many black holes (BH) with massive main-sequence dwarf companions (OB+BH binaries) are expected to be detected as binaries in DR3 and at the end of the nominal 5-yr mission (DR4). We estimate the fraction of identifiable OB+BH binaries and discuss the distributions of the masses of both components and the orbital periods. We study the impact of different BH-formation scenarios. Using tailored models for the massive star population, which assume a direct collapse and no kick upon BH formation (the fiducial case), we estimate the fraction of OB+BH systems that Gaia will detect as binaries. A distance distribution according to that of the second Alma Luminous Star catalogue (ALSII) is assumed. We investigate how many of the systems detected as binaries are identifiable as OB+BH binaries, using a method based on astrometric data. In the fiducial case we conservatively estimate that 77% of the OB+BH binaries in ALSII will be detected as binaries in DR3, of which 89% are identifiable as OB+BH binaries. This leads to a total of around 190 OB+BH binaries, a 20-fold increase in the known sample of OB+BH binaries, covering an uncharted parameter space of long-period binaries. The size and properties of the identifiable OB+BH population will contain crucial observational constraints to improve our understanding of BH formation. In DR4, the detected fraction will increase to 85%, of which 82% will be identifiable. Hence, an additional ~5 systems could be identified, which are expected to have either very short or long periods. The fractions become smaller for different BH-formation scenarios. (truncated)

==> NewCommands.tex <==
% Must be used in math mode
\newcommand{\Teff}{T_{\text{eff}}}
\newcommand{\Mini}{M_{\text{initial}}}
\newcommand{\Modot}{M_{\odot}}
\newcommand{\MSun}{M_{\odot}}
\newcommand{\Rodot}{R_{\odot}}
\newcommand{\RSun}{R_{\odot}}

\newcommand{\logL}{\log(L/L_{\odot})}

\newcommand{\LC}{_{\text{LC}}}
\newcommand{\BH}{_{\text{BH}}}

\newcommand{\kms}{km\,s$^{-1}$}

% Easy for quickly writing Table/Section/Figure \ref
\newcommand{\Tabref}{Table\,\ref}
\newcommand{\Figref}{Fig.\,\ref}
\newcommand{\Secref}{Sect.\,\ref}
\newcommand{\Eqref}{Eq.\,\eqref}
\newcommand{\Tabrefs}{Tables \ref}
\newcommand{\Figrefs}{Figs. \ref}
\newcommand{\Secrefs}{Sections \ref}
\newcommand{\nextline}{\\\indent}

\newcommand{\Gaia}{\textit{Gaia}}
\newcommand{\Gaias}{\textit{Gaia}\space}

\newcommand{\Cite}{\textcolor{red}{cite}}



% \newcommand{\aap}{Astronomy \& Astrophysics}
% \newcommand{\apj}{Astrophysical Journal}
% \newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
% \newcommand{\actaa}{Acta Astronomica}
% \newcommand{\apjl}{The Astrophysical Journal Letters}
% \newcommand{\nat}{Nature}
% \newcommand{\mnras}{Monthly Notices of the Royal Astronomical Society}
% \newcommand{\pasp}{Publications of the Astronomical Society of the Pacific}
% \newcommand{\vila}{Villanova University, dept. of Astronomy and Astrophysics}
% \newcommand{\aaps}{Astronomy and Astrophysics Supplement}
% \newcommand{\prl}{Physical Review Letters}
% \newcommand{\apjs}{The Astrophysical Journal Supplement Series}
% \newcommand{\aj}{The Astronomical Journal}
% \newcommand{\pasp}{The Publications of the Astronomical Society of the Pacific}
% \newcommand{\pasj}{Publications of the Astronomical Society of Japan}
% \newcommand{\procspie}{Proc. SPIE}
% \newcommand{\nar}{New Astronomy Reviews}

==> other_environments.tex <==
% \subsection{Going to other environments}
% \textcolor{red}{Depending on what happens in this paper with LMC and SMC results...}\\\
% With the method described above, it is straightforward to apply these corrections for any other environment with a different metallicity. Hence, we can transform the simulations to represent systems in the Small Magellanic Cloud. For this, we used $Z_{\text{SMC}} = 0.003$, such that the scaling factor becomes $0.5^{0.83}$.\nextline
\textcolor{red}{Talk about LMC and SMC or not? If yes: rewrite, because distance is not taken into account with extinction in MCs} The extinction in the LMC is calculated using $A_V = 0.3$ \citep{Imara_2007}, yielding $A_G = 0.237$. For the SMC, we used $A_G = 0.28$ \citep{Schootemeijer_2021}.
The absolute and apparent magnitudes are shown in the right panel of \Figref{fig_distances_magnitudes}. The \Gaias magnitude limits are also shown. It can readily be seen that quite a few systems will not be detected based on this magnitude limits.
